NTTSuite: Number Theoretic Transform Benchmarks for Accelerating Encrypted Computation

Privacy concerns have thrust privacy-preserving computation into the spotlight. Homomorphic encryption (HE) is a cryptographic system that enables computation to occur directly on encrypted data, providing users with strong privacy (and security) guarantees while using the same services they enjoy today unprotected. While promising, HE has seen little adoption due to extremely high computational overheads, rendering it impractical. Homomorphic encryption (HE) is a cryptographic system that enables computation to occur directly on encrypted data. In this paper we develop a benchmark suite, named NTTSuite, to enable researchers to better address these overheads by studying the primary source of HE's slowdown: the number theoretic transform (NTT). NTTSuite constitutes seven unique NTT algorithms with support for CPUs (C++), GPUs (CUDA), and custom hardware (Catapult HLS).In addition, we propose optimizations to improve the performance of NTT running on FPGAs. We find our implementation outperforms the state-of-the-art by 30%.

==> ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{GDPR}
\BIBentryALTinterwordspacing
``General data protection regulation,'' 2016, legislature 2016/679. [Online].
  Available: \url{https://gdpr-info.eu/}
\BIBentrySTDinterwordspacing

\bibitem{fb5b}
\BIBentryALTinterwordspacing
``Ftc imposes \$5 billion penalty and sweeping new privacy restrictions on
  facebook,'' 2019. [Online]. Available:
  \url{https://www.ftc.gov/news-events/press-releases/2019/07/ftc-imposes-5-billion-penalty-sweeping-new-privacy-restrictions}
\BIBentrySTDinterwordspacing

\bibitem{Spectre_Kocher2019}
P.~Kocher, J.~Horn, A.~Fogh, D.~Genkin, D.~Gruss, W.~Haas, M.~Hamburg, M.~Lipp,
  S.~Mangard, T.~Prescher, M.~Schwarz, and Y.~Yarom, ``Spectre attacks:
  Exploiting speculative execution,'' in \emph{2019 IEEE Symposium on Security
  and Privacy (SP)}, 2019, pp. 1--19.

\bibitem{meltdownattack}
\BIBentryALTinterwordspacing
``Meltdown and spectre,'' 2018. [Online]. Available:
  \url{https://meltdownattack.com/}
\BIBentrySTDinterwordspacing

\bibitem{PEC}
\BIBentryALTinterwordspacing
``Privacy-enhancing cryptography.'' [Online]. Available:
  \url{https://csrc.nist.gov/projects/pec}
\BIBentrySTDinterwordspacing

\bibitem{cheetah}
B.~Reagen, W.~Choi, Y.~Ko, V.~Lee, G.-Y. Wei, H.-H.~S. Lee, and D.~Brooks,
  ``Cheetah: Optimizing and accelerating homomorphic encryption for private
  inference,'' 2020.

\bibitem{heax}
M.~S. Riazi, K.~Laine, B.~Pelton, and W.~Dai, ``Heax: An architecture for
  computing on encrypted data,'' 2020.

\bibitem{pease}
M.~C. Pease, ``An adaptation of the fast fourier transform for parallel
  processing,'' \emph{J. ACM}, vol.~15, pp. 252--264, 1968.

\bibitem{flat}
K.~Kawamura, M.~Yanagisawa, and N.~Togawa, ``A loop structure optimization
  targeting high-level synthesis of fast number theoretic transform,'' in
  \emph{2018 19th International Symposium on Quality Electronic Design
  (ISQED)}, 2018, pp. 106--111.

\bibitem{ozcan_aysu_2020}
E.~Ozcan and A.~Aysu, ``High-level synthesis of number-theoretic transform: A
  case study for future cryptosystems,'' \emph{IEEE Embedded Systems Letters},
  vol.~12, no.~4, p. 133–136, 2020.

\bibitem{modularReduction}
\BIBentryALTinterwordspacing
A.~R.~Omondi, \emph{Modular Reduction}.\hskip 1em plus 0.5em minus 0.4em\relax
  Cham: Springer International Publishing, 2020, pp. 105--141. [Online].
  Available: \url{https://doi.org/10.1007/978-3-030-34142-8\_4}
\BIBentrySTDinterwordspacing

\bibitem{CPU_Microsoft2016}
P.~Longa and M.~Naehrig, ``Speeding up the number theoretic transform for
  faster ideal lattice-based cryptography,'' in \emph{Cryptology and Network
  Security}, S.~Foresti and G.~Persiano, Eds.\hskip 1em plus 0.5em minus
  0.4em\relax Cham: Springer International Publishing, 2016, pp. 124--139.

\bibitem{CPU_Seiler18}
G.~Seiler, ``Faster avx2 optimized ntt multiplication for ring-lwe lattice
  cryptography,'' 2018, report 2018/039.

\bibitem{HEXL2021}
\BIBentryALTinterwordspacing
F.~Boemer, S.~Kim, G.~Seifu, F.~D.~M. de~Souza, and V.~Gopal, ``Intel {HEXL:}
  accelerating homomorphic encryption with intel {AVX512-IFMA52},''
  \emph{CoRR}, vol. abs/2103.16400, 2021. [Online]. Available:
  \url{https://arxiv.org/abs/2103.16400}
\BIBentrySTDinterwordspacing

\bibitem{Barret_1987}
P.~Barrett, ``Implementing the rivest shamir and adleman public key encryption
  algorithm on a standard digital signal processor,'' in \emph{Advances in
  Cryptology --- CRYPTO' 86}, A.~M. Odlyzko, Ed.\hskip 1em plus 0.5em minus
  0.4em\relax Berlin, Heidelberg: Springer Berlin Heidelberg, 1987, pp.
  311--323.

\bibitem{MR_Yanik2002}
T.~Yanik, E.~Savas, and C.~Koc, ``Incomplete reduction in modular arithmetic,''
  in \emph{IEE Proceedings - Computers and Digital Techniques}, vol. 149,
  no.~2, 2002, pp. 46--52.

\bibitem{Longa2016}
P.~Longa and M.~Naehrig, ``Speeding up the number theoretic transform for
  faster ideal lattice-based cryptography,'' Cryptology ePrint Archive, Report
  2016/504, 2016, \url{https://ia.cr/2016/504}.

\bibitem{Cooley1965}
J.~W. Cooley and J.~W. Tukey, ``{An Algorithm for the Machine Calculation of
  Complex Fourier Series},'' \emph{Math. Comput.}, vol.~19, pp. 297--301, 1965.

\bibitem{DIF}
H.~Murakami, ``Real-valued decimation-in-time and decimation-in-frequency
  algorithms,'' \emph{IEEE Transactions on Circuits and Systems II: Analog and
  Digital Signal Processing}, vol.~41, no.~12, pp. 808--816, 1994.

\bibitem{Cochran1967}
W.~Cochran, J.~Cooley, D.~Favin, H.~Helms, R.~Kaenel, W.~Lang, G.~Maling,
  D.~Nelson, C.~Rader, and P.~Welch, ``What is the fast fourier transform?''
  \emph{Proceedings of the IEEE}, vol.~55, no.~10, pp. 1664--1674, 1967.

\bibitem{sixstep}
D.~Takahashi, \emph{High-Performance FFT Algorithms}, 10 2019, pp. 41--68.

\bibitem{GPU_Ozgun2021}
O.~Ozerk, C.~Elgezen, A.~C. Mert, E.~Ozturk, and E.~Savas, ``Efficient number
  theoretic transform implementation on gpu for homomorphic encryption,''
  Cryptology ePrint Archive, Report 2021/124, 2021,
  \url{https://ia.cr/2021/124}.

\bibitem{SHEonGPU_Badawi2018}
\BIBentryALTinterwordspacing
A.~A. Badawi, B.~Veeravalli, C.~F. Mun, and K.~M.~M. Aung, ``High-performance
  fv somewhat homomorphic encryption on gpus: An implementation using cuda,''
  \emph{IACR Transactions on Cryptographic Hardware and Embedded Systems}, vol.
  2018, no.~2, p. 70–95, May 2018. [Online]. Available:
  \url{https://tches.iacr.org/index.php/TCHES/article/view/875}
\BIBentrySTDinterwordspacing

\bibitem{Kim2020}
S.~Kim, W.~Jung, J.~Park, and J.~H. Ahn, ``Accelerating number theoretic
  transformations for bootstrappable homomorphic encryption on gpus,'' in
  \emph{2020 IEEE International Symposium on Workload Characterization
  (IISWC)}, 2020, pp. 264--275.

\bibitem{FPGA_HE_Sinha2019}
S.~S. Roy, F.~Turan, K.~Jarvinen, F.~Vercauteren, and I.~Verbauwhede,
  ``Fpga-based high-performance parallel architecture for homomorphic computing
  on encrypted data,'' Cryptology ePrint Archive, Report 2019/160, 2019,
  \url{https://ia.cr/2019/160}.

\bibitem{Nejatollahi2020}
H.~Nejatollahi, S.~Shahhosseini, R.~Cammarota, and N.~Dutt, ``Exploring energy
  efficient quantum-resistant signal processing using array processors,'' in
  \emph{ICASSP 2020 - 2020 IEEE International Conference on Acoustics, Speech
  and Signal Processing (ICASSP)}, 2020, pp. 1539--1543.

\bibitem{FPGA_Ye2021}
T.~Ye, Y.~Yang, S.~R. Kuppannagari, R.~Kannan, and V.~K. Prasanna, ``Fpga
  acceleration of number theoretic transform,'' in \emph{High Performance
  Computing}, B.~L. Chamberlain, A.-L. Varbanescu, H.~Ltaief, and P.~Luszczek,
  Eds.\hskip 1em plus 0.5em minus 0.4em\relax Cham: Springer International
  Publishing, 2021, pp. 98--117.

\bibitem{samardzic2021f1}
N.~Samardzic, A.~Feldmann, A.~Krastev, S.~Devadas, R.~Dreslinski, C.~Peikert,
  and D.~Sanchez, ``F1: A fast and programmable accelerator for fully
  homomorphic encryption,'' in \emph{MICRO-54: 54th Annual IEEE/ACM
  International Symposium on Microarchitecture}, 2021, pp. 238--252.

\bibitem{soni2023rpu}
D.~Soni, N.~Neda, N.~Zhang, B.~Reynwar, H.~Gamil, B.~Heyman, M.~Nabeel,
  A.~Al~Badawi, Y.~Polyakov, K.~Canida \emph{et~al.}, ``Rpu: The ring
  processing unit,'' in \emph{2023 IEEE International Symposium on Performance
  Analysis of Systems and Software (ISPASS)}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2023, pp. 272--282.

\bibitem{samardzic2022craterlake}
N.~Samardzic, A.~Feldmann, A.~Krastev, N.~Manohar, N.~Genise, S.~Devadas,
  K.~Eldefrawy, C.~Peikert, and D.~Sanchez, ``Craterlake: a hardware
  accelerator for efficient unbounded computation on encrypted data,'' in
  \emph{Proceedings of the 49th Annual International Symposium on Computer
  Architecture}, 2022, pp. 173--187.

\bibitem{kim2022bts}
S.~Kim, J.~Kim, M.~J. Kim, W.~Jung, J.~Kim, M.~Rhu, and J.~H. Ahn, ``Bts: An
  accelerator for bootstrappable fully homomorphic encryption,'' in
  \emph{Proceedings of the 49th Annual International Symposium on Computer
  Architecture}, 2022, pp. 711--725.

\end{thebibliography}

